Comparing and Combining Approximate Computing Frameworks

Approximate computing frameworks configure applications so they can operate at a range of points in an accuracy-performance trade-off space. Prior work has introduced many frameworks to create approximate programs. As approximation frameworks proliferate, it is natural to ask how they can be compared and combined to create even larger, richer trade-off spaces. We address these questions by presenting VIPER and BOA. VIPER compares trade-off spaces induced by different approximation frameworks by visualizing performance improvements across the full range of possible accuracies. BOA is a family of exploration techniques that quickly locate Pareto-efficient points in the immense trade-off space produced by the combination of two or more approximation frameworks. We use VIPER and BOA to compare and combine three different approximation frameworks from across the system stack, including: one that changes numerical precision, one that skips loop iterations, and one that manipulates existing application parameters. Compared to simply looking at Pareto-optimal curves, we find VIPER's visualizations provide a quicker and more convenient way to determine the best approximation technique for any accuracy loss. Compared to a state-of-the-art evolutionary algorithm, we find that BOA explores 14x fewer configurations yet locates 35% more Pareto-efficient points.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDFLATEX=pdflatex
BIBTEX=bibtex

FIG-FILES = figs/*.png img/*.tex
TEX-FILES = *.tex
BIB-FILES = *.bib
TOP-LEVEL-ROOT = paper


#SAMPLES = paper.tex 

#PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${TOP-LEVEL-ROOT}.pdf


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	$(PDFLATEX) -shell-escape $<
	- $(BIBTEX) $*
	$(PDFLATEX) -shell-escape $<
	$(PDFLATEX) -shell-escape $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do $(PDFLATEX) $<; done

paper.pdf: ${TEX-FILES}

#paper.pdf: ${TEX-FILES} ${BIB-FILES} ${FIG-FILES} 
#	$(PDFLATEX) -shell-escape ${TOP-LEVEL-ROOT}
#	$(BIBTEX) ${TOP-LEVEL-ROOT}
#	$(PDFLATEX) -shell-escape ${TOP-LEVEL-ROOT}


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.pdf

squeaky:
	$(RM) out/*

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.


==> img/cs1viperLines/App-cs1viperLine.tex <==
\zse{mps={msze=0.5p}}
\pfplsse{syle={se,y}}
\pfplsse{msyle={se,e}}
\pfplsse{mjsyle={e,ee!50!l}}
\pfplsse{eveyxlel/.ppesyle={f=\spsze,ysf=0.5ex}}
\pfplsse{eveyylel/.ppesyle={f=\spsze,xsf=0.5ex}}

\pfplsse{eveym/.ppesyle={lew=0.4p}}

\pfplsse{eveyxs/.ppesyle={f=\spsze}}

\ewmm{\xse}{0.99}

\e{zpe}[]
\e{ee}

%\fflse
\e{xs}[
le={\smll{App}},
lesyle={ysf=-0.5em},
xlel={AyLss},
ylel={PIR},
xlelsyle={ysf=0.6em},
ylelsyle={ysf=-0.5em},
xm=0,xmx=0.5,
ym=0,ymx=1,
x={0,0.1,0.2,0.3,0.4,0.5},
xlels={0,0.1,0.2,0.3,0.4,0.5},
y={0,0.2,0.4,0.6,0.8,1},
ylels={0,0.2,0.4,0.6,0.8,1},
leeps=es,
w=0.22\exw,
%ymjs=e,
syle=se,
]


\e{spe}[lye]
	\fll[ee,py=0.2]({elxss:0,\xse})ele({elxss:1,1});
	\fll[e,py=0.2]({elxss:0,0})ele({elxss:1,\xse});
%\w[l_le,](xss:0,\xse)--(xss:1,\xse);
	\fll[l_le,py=1]({elxss:0,\xse-0.002})ele({elxss:1,\xse+0.002});
\e{spe}


\pl[l=l_le,lew=1.2p]le[xex=0,yex=1,lsep=mm]{m/D/vpeLes//pefImpvLe-App-LP.sv};
\pl[l=l_e,lew=1.2p]le[xex=0,yex=1,lsep=mm]{m/D/vpeLes//pefImpvLe-App-SK.sv};
\pl[l=l_ee,lew=1.2p]le[xex=0,yex=1,lsep=mm]{m/D/vpeLes//pefImpvLe-App-AML.sv};

%\lee{LP,SK,AML}

\e{xs}

%\f
\e{ee}
\e{zpe}


==> img/cs3viperLines/Fluidanimate-cs3viperLine.tex <==
\tikzset{mark options={mark size=0.5 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}

\newcommand{\axisheight}{0.54408}

\begin{tikzpicture} [tight background]
\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Fluidanimate}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={PIR},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=0.9,
        ymin=0, ymax=1,
        xtick={0,0.3,0.6,0.9},
        xticklabels={0,0.3,0.6,0.9},
        ytick={0,0.2,0.4,0.6,0.8,1},
        yticklabels={0,0.2,0.4,0.6,0.8,1},
        legend style={at={(1.8,0.650)},anchor=north east},
        width=0.35\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
    ]


        \begin{scope}[on background layer]
           \fill[color_black,opacity=0.4] ({axis cs:0,0}) rectangle ({axis cs:0.029895,1});
           \fill[color_navy,opacity=0.4] ({axis cs:0.029895,0}) rectangle ({axis cs:0.44543,1});
           \fill[color_black,opacity=0.4] ({axis cs:0.44543,0}) rectangle ({rel axis cs:1,1});
	 % \fill[green,opacity=0.2] ({rel axis cs:0,\axisheight}) rectangle ({rel axis cs:1,1});
  	  %\fill[red,opacity=0.2] ({rel axis cs:0,0}) rectangle ({rel axis cs:1,1});
    %\draw[color_blue, thick] (axis cs:0,\axisheight) -- (axis cs:1,\axisheight);    
  	 % \fill[color_blue,opacity=1] ({rel axis cs:0,\axisheight-0.002}) rectangle ({rel axis cs:1,\axisheight+0.002});
    \end{scope}
   

    \addplot[color=color_orange, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/testCS3/perfImprovLine-Fluidanimate-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/testCS3/perfImprovLine-Fluidanimate-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/testCS3/perfImprovLine-Fluidanimate-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/testCS3/perfImprovLine-Fluidanimate-BOA-2.csv};
    \addplot[color=color_navy, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/testCS3/perfImprovLine-Fluidanimate-BOA-5.csv};
    \addplot[color=color_black, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/testCS3/perfImprovLine-Fluidanimate-BOA-10.csv};


    \legend{MCKP, NSGA, BOA(TH=0.0), BOA(TH=0.02), BOA(TH=0.05), BOA(TH=0.10)}


    %\legend{LP, SK, AML}  
    
    \end{axis}

    %\fi 
\end{centering}
\end{tikzpicture}


==> img/exhconfigSpace/Blackscholes-configSpace.tex <==
\tikzset{mark options={mark size=0.5 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}



\begin{tikzpicture} 
\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Blackscholes}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={Normalized Runtime},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=0.5,
        ymin=0.94, ymax=1,
        xtick={0,0.1,0.2,0.3,0.4,0.5},
        xticklabels={0,0.1,0.2,0.3,0.4,0.5},
        ytick={0.94,0.96,0.98,1},
        yticklabels={0.94,0.96,0.98,1},
        legend pos=north west,
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
    ]


    \addplot[color=color_orange, line width=1.2pt ,mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/test/paretoLine-Blackscholes-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt ,mark=square*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/test/paretoLine-Blackscholes-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt ,mark=triangle*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/test/paretoLine-Blackscholes-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt ,mark=diamond*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/test/paretoLine-Blackscholes-BOA-2.csv};
    \addplot[color=color_navy, line width=1.2pt ,mark=otimes*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/test/paretoLine-Blackscholes-BOA-5.csv};
    
    


    %\addplot[scatter, scatter/use mapped color={draw=color_blue,fill=color_blue}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Blackscholes-LP.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_red,fill=color_red}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Blackscholes-SK.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_green,fill=color_green}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Blackscholes-AML.csv};
    

    %\addplot[color=blue,mark=square,]coordinates {(0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)};\legend{CuSO$_4\cdot$5H$_2$O}  
    
    \end{axis}

    %\fi 
\end{centering}
\end{tikzpicture}

\noindent\demofig
\vspace{-5.0em}

==> img/exhconfigSpace/Canneal-configSpace.tex <==
\tikzset{mark options={mark size=1.0 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}


\hspace*{-37pt}


\begin{tikzpicture} 
%\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Canneal}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={Normalized Runtime},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=0.3,
        ymin=0.4, ymax=1,
        xtick={0,0.1,0.2,0.30},
        xticklabels={0,0.1,0.2,0.30},
        ytick={0.4,0.6,0.8,1},
        yticklabels={0.4,0.6,0.8,1},
        legend pos=north west,
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
    ]


    \addplot[color=color_orange, line width=1.2pt ,mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Canneal-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt ,mark=triangle*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Canneal-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt ,mark=square*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Canneal-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt ,mark=diamond*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Canneal-BOA-5.csv};
    \addplot[color=color_navy, line width=1.2pt ,mark=pentagon*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Canneal-BOA-Randomized.csv};
    \addplot[color=color_black, line width=1.2pt ,mark=10-pointed star] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Canneal-exhaustive.csv};
    

    %\addplot[scatter, scatter/use mapped color={draw=color_blue,fill=color_blue}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Canneal-LP.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_red,fill=color_red}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Canneal-SK.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_green,fill=color_green}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Canneal-AML.csv};
    

    %\addplot[color=blue,mark=square,]coordinates {(0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)};\legend{CuSO$_4\cdot$5H$_2$O}  
    
    \end{axis}

    %\fi 
%\end{centering}
\end{tikzpicture}

\noindent\demofig
\vspace{-5.0em}

==> img/exhconfigSpace/Fluidanimate-configSpace.tex <==
\tikzset{mark options={mark size=1.0 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}


\hspace*{-37pt}


\begin{tikzpicture} 
%\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Fluidanimate}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={Normalized Runtime},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=0.6,
        ymin=0, ymax=1,
        xtick={0,0.1,0.2,0.3,0.4,0.5,0.6},
        xticklabels={0,0.1,0.2,0.3,0.4,0.5,0.6},
        ytick={0,0.2,0.4,0.6,0.8,1},
        yticklabels={0,0.2,0.4,0.6,0.8,1},
        legend pos=north west,
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
    ]


    \addplot[color=color_orange, line width=1.2pt ,mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Fluidanimate-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt ,mark=triangle*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Fluidanimate-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt ,mark=square*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Fluidanimate-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt ,mark=diamond*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Fluidanimate-BOA-5.csv};
    \addplot[color=color_navy, line width=1.2pt ,mark=pentagon*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Fluidanimate-BOA-Randomized.csv};
    \addplot[color=color_black, line width=1.2pt ,mark=10-pointed star] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Fluidanimate-exhaustive.csv};
    

    %\addplot[scatter, scatter/use mapped color={draw=color_blue,fill=color_blue}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Fluidanimate-LP.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_red,fill=color_red}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Fluidanimate-SK.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_green,fill=color_green}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Fluidanimate-AML.csv};
    

    %\addplot[color=blue,mark=square,]coordinates {(0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)};\legend{CuSO$_4\cdot$5H$_2$O}  
    
    \end{axis}

    %\fi 
%\end{centering}
\end{tikzpicture}

\noindent\demofig
\vspace{-5.0em}

==> img/exhconfigSpace/Kmeans-configSpace.tex <==
\tikzset{mark options={mark size=1.0 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}


\hspace*{-37pt}


\begin{tikzpicture} 
%\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Kmeans}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={Normalized Runtime},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=5,
        ymin=0, ymax=1,
        xtick={0,1,2,3,4,5},
        xticklabels={0,1,2,3,4,5},
        ytick={0,0.2,0.4,0.6,0.8,1},
        yticklabels={0,0.2,0.4,0.6,0.8,1},
        legend style={at={(2.00,1.00)},anchor=north east},
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
    ]


    \addplot[color=color_orange, line width=1.2pt ,mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Kmeans-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt ,mark=triangle*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Kmeans-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt ,mark=square*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Kmeans-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt ,mark=diamond*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Kmeans-BOA-5.csv};
    \addplot[color=color_navy, line width=1.2pt ,mark=pentagon*] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Kmeans-BOA-Randomized.csv};
    \addplot[color=color_black, line width=1.2pt ,mark=10-pointed star] table[x index=0,y index=1,col sep=comma] {img/Data/paretoLines/exhpc/paretoLine-Kmeans-exhaustive.csv};
    
    

    %\addplot[scatter, scatter/use mapped color={draw=color_blue,fill=color_blue}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Kmeans-LP.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_red,fill=color_red}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Kmeans-SK.csv};
    %\addplot[scatter, scatter/use mapped color={draw=color_green,fill=color_green}, only marks, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/tradeoffSpace/train/tradeoffSpace-Kmeans-AML.csv};
    

    \legend{MCKP, NSGA, BOA-simple, BOA-flex, BOA-prob, Exhaustive}


    %\addplot[color=blue,mark=square,]coordinates {(0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)};\legend{CuSO$_4\cdot$5H$_2$O}  
    
    \end{axis}

    %\fi 
%\end{centering}
\end{tikzpicture}

\noindent\demofig
\vspace{-5.0em}

==> img/exhviperLines/Blackscholes-exhviperLine.tex <==
\tikzset{mark options={mark size=0.5 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}

\newcommand{\axisheight}{0.54408}

\begin{tikzpicture} 
\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Blackscholes}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={PIR},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=0.5,
        ymin=0, ymax=1,
        xtick={0,0.10,0.20,0.30,0.40,0.50},
        xticklabels={0,0.10,0.20,0.30,0.40,0.50},
        ytick={0,0.2,0.4,0.6,0.8,1},
        yticklabels={0,0.2,0.4,0.6,0.8,1},
        legend pos=north east,
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
    ]


        \begin{scope}[on background layer]

              \fill[color_navy,opacity=0.4] ({axis cs:0,0}) rectangle ({rel axis cs:1,1});

	 % \fill[green,opacity=0.4] ({rel axis cs:0,\axisheight}) rectangle ({rel axis cs:1,1});
  	  %\fill[red,opacity=0.4] ({rel axis cs:0,0}) rectangle ({rel axis cs:1,1});
    %\draw[color_blue, thick] (axis cs:0,\axisheight) -- (axis cs:1,\axisheight);    
  	 % \fill[color_blue,opacity=1] ({rel axis cs:0,\axisheight-0.002}) rectangle ({rel axis cs:1,\axisheight+0.002});
    \end{scope}
   

    \addplot[color=color_orange, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/test/perfImprovLine-Blackscholes-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/test/perfImprovLine-Blackscholes-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/test/perfImprovLine-Blackscholes-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/test/perfImprovLine-Blackscholes-BOA-2.csv};
    \addplot[color=color_navy, line width=1.2pt] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/test/perfImprovLine-Blackscholes-BOA-5.csv};



    %\legend{LP, SK, AML}  
    
    \end{axis}

    %\fi 
\end{centering}
\end{tikzpicture}


==> img/exhviperLines/Canneal-exhviperLine.tex <==
\tikzset{mark options={mark size=1.0 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}

\newcommand{\axisheight}{0.54408}

\hspace*{-37pt}

\begin{tikzpicture} 
%\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Canneal}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={PIR},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=0.28,
        ymin=0, ymax=1,
        xtick={0,0.07,0.14,0.21,0.28},
        xticklabels={0,0.07,0.14,0.21,0.28},
        ytick={0,0.2,0.4,0.6,0.8,1},
        yticklabels={0,0.2,0.4,0.6,0.8,1},
        legend pos=north east,
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
        mark repeat={100}
    ]


        \begin{scope}[on background layer]
                      \fill[color_black,opacity=0.4] ({axis cs:0,0}) rectangle ({rel axis cs:1,1});

     % \fill[green,opacity=0.4] ({rel axis cs:0,\axisheight}) rectangle ({rel axis cs:1,1});
      %\fill[red,opacity=0.4] ({rel axis cs:0,0}) rectangle ({rel axis cs:1,1});
    %\draw[color_blue, thick] (axis cs:0,\axisheight) -- (axis cs:1,\axisheight);    
     % \fill[color_blue,opacity=1] ({rel axis cs:0,\axisheight-0.002}) rectangle ({rel axis cs:1,\axisheight+0.002});
    \end{scope}
   

    \addplot[color=color_orange, line width=1.2pt, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Canneal-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt, mark=triangle*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Canneal-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt, mark=square*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Canneal-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt, mark=diamond*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Canneal-BOA-5.csv};
    \addplot[color=color_navy, line width=1.2pt, mark=pentagon*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Canneal-BOA-Rand.csv};
    \addplot[color=color_black, line width=1.2pt, mark=10-pointed star] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Canneal-exhaustive.csv};


    %\legend{LP, SK, AML}  
    
    \end{axis}

    %\fi 
%\end{centering}
\end{tikzpicture}


\noindent\demofig
\vspace{-5.0em}

==> img/exhviperLines/Fluidanimate-exhviperLine.tex <==
\tikzset{mark options={mark size=1.0 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}

\newcommand{\axisheight}{0.54408}

\hspace*{-37pt}

\begin{tikzpicture} 
%\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Fluidanimate}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={PIR},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=0.6,
        ymin=0, ymax=1,
        xtick={0,0.1,0.2,0.3,0.4,0.5,0.6},
        xticklabels={0,0.1,0.2,0.3,0.4,0.5,0.6},
        ytick={0,0.2,0.4,0.6,0.8,1},
        yticklabels={0,0.2,0.4,0.6,0.8,1},
        legend pos=north east,
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
        mark repeat={100}
    ]


        \begin{scope}[on background layer]
                      \fill[color_black,opacity=0.4] ({axis cs:0,0}) rectangle ({rel axis cs:1,1});

     % \fill[green,opacity=0.4] ({rel axis cs:0,\axisheight}) rectangle ({rel axis cs:1,1});
      %\fill[red,opacity=0.4] ({rel axis cs:0,0}) rectangle ({rel axis cs:1,1});
    %\draw[color_blue, thick] (axis cs:0,\axisheight) -- (axis cs:1,\axisheight);    
     % \fill[color_blue,opacity=1] ({rel axis cs:0,\axisheight-0.002}) rectangle ({rel axis cs:1,\axisheight+0.002});
    \end{scope}
   

    \addplot[color=color_orange, line width=1.2pt, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Fluidanimate-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt, mark=triangle*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Fluidanimate-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt, mark=square*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Fluidanimate-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt, mark=diamond*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Fluidanimate-BOA-5.csv};
    \addplot[color=color_navy, line width=1.2pt, mark=pentagon*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Fluidanimate-BOA-Rand.csv};
    \addplot[color=color_black, line width=1.2pt, mark=10-pointed star] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Fluidanimate-exhaustive.csv};



    %\legend{LP, SK, AML}  
    
    \end{axis}

    %\fi 
%\end{centering}
\end{tikzpicture}


\noindent\demofig
\vspace{-5.0em}

==> img/exhviperLines/Kmeans-exhviperLine.tex <==
\tikzset{mark options={mark size=1.0 pt}}
\pgfplotsset{grid style={dashed,gray}}
\pgfplotsset{minor grid style={dashed,red}}
\pgfplotsset{major grid style={dotted,green!50!black}}
\pgfplotsset{every x tick label/.append style={font=\scriptsize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\scriptsize, xshift=0.5ex}}

\pgfplotsset {every mark/.append style={line width=0.4pt}}

\pgfplotsset{every axis/.append style={font=\scriptsize}}

\newcommand{\axisheight}{0.54408}

\hspace*{-37pt}

\begin{tikzpicture} 
%\begin{centering}

    %\iffalse
    \begin{axis}[
        title={\small {Kmeans}},
        title style={yshift= -0.5em},
        xlabel={AccuracyLoss},
        ylabel={PIR},
        xlabel style={yshift= 0.6em},
        ylabel style={yshift=-0.5em},
        xmin=0, xmax=5,
        ymin=0, ymax=1,
        xtick={0,1,2,3,4,5},
        xticklabels={0,1,2,3,4,5},
        ytick={0,0.2,0.4,0.6,0.8,1},
        yticklabels={0,0.2,0.4,0.6,0.8,1},
        legend style={at={(2.00,1.00)},anchor=north east},
        width=0.26\textwidth,
        %ymajorgrids=true,
        grid style=dashed,
        mark repeat={100}
    ]


        \begin{scope}[on background layer]
                      \fill[color_black,opacity=0.4] ({axis cs:0,0}) rectangle ({rel axis cs:1,1});

     % \fill[green,opacity=0.4] ({rel axis cs:0,\axisheight}) rectangle ({rel axis cs:1,1});
      %\fill[red,opacity=0.4] ({rel axis cs:0,0}) rectangle ({rel axis cs:1,1});
    %\draw[color_blue, thick] (axis cs:0,\axisheight) -- (axis cs:1,\axisheight);    
     % \fill[color_blue,opacity=1] ({rel axis cs:0,\axisheight-0.002}) rectangle ({rel axis cs:1,\axisheight+0.002});
    \end{scope}
   

    \addplot[color=color_orange, line width=1.2pt, mark=*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Kmeans-MCKP.csv};
    \addplot[color=color_brown, line width=1.2pt, mark=triangle*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Kmeans-NSGA.csv};
    \addplot[color=color_pink, line width=1.2pt, mark=square*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Kmeans-BOA-0.csv};
    \addplot[color=color_purple, line width=1.2pt, mark=diamond*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Kmeans-BOA-5.csv};
    \addplot[color=color_navy, line width=1.2pt, mark=pentagon*] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Kmeans-BOA-Rand.csv};
    \addplot[color=color_black, line width=1.2pt, mark=10-pointed star] table[x index=0,y index=1,col sep=comma] {img/Data/viperLines/exhpc/perfImprovLine-Kmeans-exhaustive.csv};

    \legend{MCKP, NSGA, BOA-simple, BOA-flex, BOA-prob, Exhaustive}


    %\legend{LP, SK, AML}  
    
    \end{axis}

    %\fi 
%\end{centering}
\end{tikzpicture}


\noindent\demofig
\vspace{-5.0em}
